Renormalization of a Contact Interaction on a Lattice

Contact interactions can be used to describe a system of particles at unitarity, contribute to the leading part of nuclear interactions and are numerically non-trivial because they require a proper regularization and renormalization scheme. We explain how to tune the coefficient of a contact interaction between non-relativistic particles on a discretized space in 1, 2, and 3 spatial dimensions such that we can remove all discretization artifacts. By taking advantage of a latticized L\"uscher zeta function, we can achieve a momentum-independent scattering amplitude at any finite lattice spacing.

==> section/continuum-extrapolation.tex <==
\section{Continuum extrapolation}\label{sec:continuum}

\begin{figure}[ht!]
\center
\input{figure/a1g-state-overlap.pgf}
\caption{A1g state ovelap\label{fig:a1g-state-overlap}}
\end{figure}


\begin{figure}[ht!]
\center
\input{figure/continuum-spectrum_a-inv_+0.0_zeta_spherical_projector_a1g_n-eigs_200.pgf}
\caption{A1g state ovelap\label{fig:a1g-state-overlap}}
\end{figure}


==> section/results.tex <==
\section{Results}

We begin our discussion with L\"uscher's formalism in both three dimensions and one dimension.  Aside from the obvious change in units and reduced dimensionality when going from three to one dimension, the technical aspects of either case are similar enough that there is no reason to discuss them separately.  On the other hand, there are subtle technical issues leading to large differences in two dimensions, and so we reserve the discussion of L\"uscher's formalism in two dimensions in a subsequent section.

\input{section/results/three-dimensions}
\input{section/results/one-dimension}
\input{section/results/two-dimensions}


==> section/two-dimensions/scale-invariance.tex <==
\subsection{The scale invariant limit in 2 dimensions}

In the spirit of Nussinov and Nussinov~\cite{nussinov2004bcs}, Nishida and Son~\cite{Nishida:2006eu} analyzed the two-dimensional unitary limit (or near it) by investigating the system in $2+\epsilon$ dimensions, using $\epsilon$ as a perturbative parameter (not to be confused with the lattice spacing).
They found the trivial solution in the scale-invariant limit; namely, the two-body system becomes non-interacting as the scattering length $\tilde a_{20} \goesto\infty$.
Our results also show this behavior, since, for fixed $L$, the intersection of a flat scattering amplitude given by $\tilde a_{20}$ goes to the non-interacting finite-volume energies as the scattering length grows large with either sign, indicating a trivial theory, as seen in \Figref{luescher2d}.

In exactly two dimensions, however, the logarithmic dependence of the scattering length requires an accompanying scale so as to make the argument of the logarithm dimensionless, a consequence of the fact that in 2 dimensions, the interaction parameters of the Schr\"odinger equation are dimensionless.
\emph{Dimensionful} observables occur via dimensional transmutation \cite{} which requires some fiducial external scale, which in any finite-volume calculation is naturally given by the size of the volume.
Thus the scale-invariant limit becomes sensitive to the order in which one takes either $\tilde a_{20}\goesto\infty$ and $L\goesto\infty$ limits.
Taking either limit first, indpendently of the other, will give the trivial scale-invariant limit found in \cite{Nishida:2006eu}.
However, there is a particular limit in which the scale-invariant system gives non-trivial solutions.
To see this, note that when $\tilde a_{20}=\frac{L}{2\pi}$ the finite-volume energies must zero the zeta function in the quanization condition~\eqref{2d luscher}, as in three dimensions when $a_{30}\to\infty$ and one dimension when $a_{10}\to 0$.

In those dimensions, such a situation is akin to the unitary limit, once the infinite volume limit has been taken.
This limit can be done independently of taking $a_{30}\to\infty$ (3-D) or $a_{10}\to0$ (1-D).
However, in two dimensions, because of the logarithmic dependence, demanding that the zeta function remains zeroed axis requires the infinite volume limit $L\to\infty$ taken together with $\tilde a_{20}$.
In particular, for the \emph{non-trivial} scale-invariant limit, one must take both $\tilde a_{20}\goesto \infty$ and $L\to\infty$ limits simultaneously \emph{such that} $L/\tilde a_{20}=2\pi$.
Such a procedure keeps the dispersion zeta function $S^{\dispersion}_2$ zeroed at each step of the extrapolation, resulting in a non-trivial, scale-invariant, two-body system in two dimensions.


==> section/two-particle-scattering/tuning-to-phase-shifts.tex <==
\subsection{Tuning to phase shifts on the lattice}\label{sec:tuning}

Observables in a FV lattice theory must converge against their physical counterpart in the IV and continuum limit.
Because the hamiltonian is implmented in a discrete finite volume, we must match the interactions to a discrete finite observable.
The implementation is well behaved if, after the matching of one observable (input), the IV and continuum limit for other observales (prediction) converges against the physical counterpart.
The implementation of the hamiltonian includes only one parameter, the strength of the contact interaction, which we match against scattering information.
The goal is to reproduce the entire phase shifts as a function of scattering momenta by matching the interactions to just one scattering momentum point.
The FV scattering spectrum can be exactly computed by using L\"{u}scher's formalism \textit{in reverse}: we compute the intersections of the phase shifts with the zeta function to extract the finit volume spectrum (see also \Figref{tuning})
\begin{equation}
    S^\spherical_D(x_i)
    =
    \frac{1}{\pi^2 L^{D-2}}
    \begin{cases}
        -\frac{1}{a_{03} \pi}   & D=3\\
        \frac{1}{\pi}\log(x_i) + \frac{2}{\pi} \log \left(\frac{ 2 \pi R_{02}}{L}\right) & D=2\\
        2 a_{01}   & D=1
    \end{cases}
	\, .
\end{equation}

We compute the FV discrete spectrum $\{E_i(\epsilon)\}$, adjust the contact interaction such that the ground state energy $E_0(\epsilon)$ matches the first zero of the zeta function $x_0 = 2 \mu E_0(\epsilon) L^2 / (2 \pi)^2$  and repeat the procedure for different lattice spacings.

